Text Augmentation in a Multi-Task View

Traditional data augmentation aims to increase the coverage of the input distribution by generating augmented examples that strongly resemble original samples in an online fashion where augmented examples dominate training. In this paper, we propose an alternative perspective -- a multi-task view (MTV) of data augmentation -- in which the primary task trains on original examples and the auxiliary task trains on augmented examples. In MTV data augmentation, both original and augmented samples are weighted substantively during training, relaxing the constraint that augmented examples must resemble original data and thereby allowing us to apply stronger levels of augmentation. In empirical experiments using four common data augmentation techniques on three benchmark text classification datasets, we find that the MTV leads to higher and more robust performance improvements than traditional augmentation.

==> fables/graphs_avg.tex <==
\pgfplotsset{width=4.05cm,height=3.5cm,compat=1.9}
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\begin{figure*}[th]
\vspace{-1.3mm}
% \begin{centering}
%
%
%
%
%
\begin{tikzpicture}
\begin{axis}[
    title={\textbf{Token Substitution}},
    title style={yshift=-1.1ex,font=\small},
    ylabel={Improvement (\%)},
    xmin=-0.03, xmax=0.53,
    ymin=-4.4, ymax=4.4,
    xtick={0, 0.2, 0.4},
    ytick={-4, -2, 0, 2, 4},
    legend pos=outer north east,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
    xlabel={Strength $\alpha$},
    x label style={at={(axis description cs:0.5,-0.18)},anchor=north,font=\small},
    y label style={at={(axis description cs:-0.22,0.5)},anchor=south,font=\small},
]
\addplot[
    color=blue,
    mark=o,
    mark size=2.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  2.1)
    (0.1,   1.47)
    (0.2,   1.97)
    (0.3,   2.07)
    (0.4,   1.47)
    (0.5,   1.87)
    };
\addplot[
    color=red,
    mark=triangle,
    mark size=3.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  1.33)
    (0.1,   1.17)
    (0.2,   0.43)
    (0.3,   0.33)
    (0.4,   -0.37)
    (0.5,   -2.63)
    };
    % \node[] at (axis cs: 10,23) {HUFF};
\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}
\begin{axis}[
    title={\textbf{Pervasive Dropout}},
    title style={yshift=-1.5ex,font=\small},
    xmin=-0.03, xmax=0.53,
    ymin=-4.4, ymax=4.4,
    xtick={0, 0.2, 0.4},
    ytick={-4, -2, 0, 2, 4},
    yticklabels={,,},
    legend pos=outer north east,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
    xlabel={Strength $\alpha$},
    x label style={at={(axis description cs:0.5,-0.18)},anchor=north,font=\small},
    y label style={at={(axis description cs:-0.27,0.5)},anchor=south,font=\small},
]
\addplot[
    color=blue,
    mark=o,
    mark size=2.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  0.93)
    (0.1,   1.53)
    (0.2,   1.97)
    (0.3,   2.27)
    (0.4,   2.53)
    (0.5,   2.43)
    };
\addplot[
    color=red,
    mark=triangle,
    mark size=3.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  0.8)
    (0.1,   1.8)
    (0.2,   1.53)
    (0.3,   1.77)
    (0.4,   0.83)
    (0.5,   -2.53)
    };
\end{axis}
\end{tikzpicture}
%
%
\begin{tikzpicture}
\begin{axis}[
    title={\textbf{Token Injection}},
    title style={yshift=-1.5ex,font=\small},
    xmin=-0.03, xmax=0.53,
    ymin=-4.4, ymax=4.4,
    xtick={0, 0.2, 0.4},
    ytick={-4, -2, 0, 2, 4},
    yticklabels={,,},
    legend pos=outer north east,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
    xlabel={Strength $\alpha$},
    x label style={at={(axis description cs:0.5,-0.18)},anchor=north,font=\small},
    y label style={at={(axis description cs:-0.27,0.5)},anchor=south,font=\small},
]
\addplot[
    color=blue,
    mark=o,
    mark size=2.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  1.4)
    (0.1,   1.27)
    (0.2,   1.73)
    (0.3,   1.9)
    (0.4,   2.13)
    (0.5,   2.17)
    };
\addplot[
    color=red,
    mark=triangle,
    mark size=3.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  0.67)
    (0.1,   0.3)
    (0.2,   0.27)
    (0.3,   0.57)
    (0.4,   -1.0)
    (0.5,   -1.53)
    };
    % \node[] at (axis cs: 10,23) {HUFF};
\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}
\begin{axis}[
    title={\textbf{Positional Shuffling}},
    title style={yshift=-1.5ex,font=\small},
    xmin=-0.03, xmax=0.53,
    ymin=-4.4, ymax=4.4,
    xtick={0, 0.2, 0.4},
    ytick={-4, -2, 0, 2, 4},
    yticklabels={,,},
    legend pos=outer north east,
    legend style={font=\small},
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
    xlabel={Strength $\alpha$},
    x label style={at={(axis description cs:0.5,-0.18)},anchor=north,font=\small},
    y label style={at={(axis description cs:-0.22,0.5)},anchor=south,font=\small},
]
\addplot[
    color=blue,
    mark=o,
    mark size=2.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  1.9)
    (0.1,   2.1)
    (0.2,   2.4)
    (0.3,   1.97)
    (0.4,   2.47)
    (0.5,   1.7)
    };
    \addlegendentry{MTV, $\gamma_\textrm{O}\shortequals0.5$}
\addplot[
    color=red,
    mark=triangle,
    mark size=3.5pt,
    ]
    coordinates {
    (0.0,   0.0)
    (0.05,  1.43)
    (0.1,   0.83)
    (0.2,   0.7)
    (0.3,   -0.27)
    (0.4,   -0.1)
    (0.5,   -1.5)
    };
    \addlegendentry{Traditional ($\gamma_\textrm{O}\shortequals0$)}
    % \node[] at (axis cs: 10,23) {HUFF};
\end{axis}
\end{tikzpicture}
%
%
%
%
%
%
%
\caption{
Performance boosts using the traditional and multi-task view (MTV) frameworks for four data augmentation techniques. 
In the traditional framework, improvements are largest when augmentation strength $\alpha$ is small, with performance deteriorating for large $\alpha$. 
The MTV, on the other hand, jointly optimizes for both original and augmented data, leveraging higher $\alpha$ to provide higher and more robust performance gains.
Per-dataset results are also shown for reference in Figure \ref{fig:graphs} in the Appendix.
}
\vspace{-1.0mm}
\label{fig:graphs-avg}
% \end{centering}
\end{figure*}
